OSKDet: Towards Orientation-sensitive Keypoint Localization for Rotated Object Detection

Rotated object detection is a challenging issue of computer vision field. Loss of spatial information and confusion of parametric order have been the bottleneck for rotated detection accuracy. In this paper, we propose an orientation-sensitive keypoint based rotated detector OSKDet. We adopt a set of keypoints to characterize the target and predict the keypoint heatmap on ROI to form a rotated target. By proposing the orientation-sensitive heatmap, OSKDet could learn the shape and direction of rotated target implicitly and has stronger modeling capabilities for target representation, which improves the localization accuracy and acquires high quality detection results. To extract highly effective features at border areas, we design a rotation-aware deformable convolution module. Furthermore, we explore a new keypoint reorder algorithm and feature fusion module based on the angle distribution to eliminate the confusion of keypoint order. Experimental results on several public benchmarks show the state-of-the-art performance of OSKDet. Specifically, we achieve an AP of 77.81% on DOTA, 89.91% on HRSC2016, and 97.18% on UCAS-AOD, respectively.

==> Experiments/Datasets/FDDB.tex <==
\cite{FDDB} is a unconstrained face dataset which contains 5171 faces in 2845 images. The annotations have horizontal rectangle and oblique ellipse two forms.
% It has two labeling forms: horizontal rectangle and oblique ellipse. 
% Mainstream models use ellipse labels for evaluation and there is no rotation box evaluation metric. 
% Since our model cannot generate ellipse predictions, we only visualize the detection results.

==> Experiments/main_result/ucas-aod.tex <==
\begin{table}[]
\centering
\scriptsize
\begin{tabular}{|l|lll|}
\hline
Method & Plane & Car   & mAP   \\ \hline
\hline
YOLOv2 & 96.60 & 79.20 & 87.90 \\
R-DFPN & 95.90 & 82.50 & 89.20 \\
DRBOX & 94.90 & 85.00 & 89.95 \\
S2 ARN & 97.60 & 92.20 & 94.90 \\
RetinaNet-H & 97.34 & 93.60 & 95.47 \\
FADet  & 98.69 & 92.72 & 95.71 \\
R3 Det  & 98.20 & 94.14 & 96.17 \\
SCRDet++  & 98.93 & 94.97 & 96.95 \\
PolarDet  & 99.08 & 94.96 & 97.02 \\ \hline
\end{tabular}
\caption{}
\label{table3}
\end{table}

==> methods/postprocess.tex <==


The network output is a heatmap representing the position probability of keypoint, which needs to be decoded to the point coordinate. Since our supervision target is a gaussian distribution heatmap, it is assumed that the generated heatmap roughly also shows a gaussian distribution. Suppose the decoded ROI is $\left(x, y, w, h)\right$, we calculate the final coordinates $\left(p_{x}, p_{y}\right)$ of each heatmap through Eq \ref{eq10}.

\begin{equation}\label{eq10}
\begin{array}{c}
p_{x}^{h}=\frac{\sum_{i=0}^{M-1} \sum_{j=0}^{M-1}(i) \cdot \sigma\left(h_{i j}\right)}{\sum_{i=0}^{M-1} \sum_{j=0}^{M-1} \sigma\left(h_{i j}\right)} ,   
p_{x}=x+p_{x}^{h} \frac{w}{M} \vspace{1ex}\\
p_{y}^{h}=\frac{\sum_{i=0}^{M-1} \sum_{j=0}^{M-1}(j) \cdot \sigma\left(h_{i j}\right)}{\sum_{i=0}^{M-1} \sum_{j=0}^{M-1} \sigma\left(h_{i j}\right)} ,  
p_{y}=y+p_{y}^{h} \frac{h}{M}
\end{array}
\end{equation}

Considering that some points may be outside the ROI boundary, we set a threshold for the confidence of the heatmap calculated by the sigmoid function. When it is less than the threshold, we consider that this point does not exist or the prediction is wrong, and discard it. Theoretically 4 points can determine a quadrilateral, but as discussed earlier, some points may not be in the ROI range, or the heatmap of multiple channels predicts the same position. We expand the point set to 8 (4 vertices and 4 midpoints) to enhance the stability of detection. Due to the complexity of the prediction circumstances, we design a simple postprocess method. First we make a polygon by the 4 points (4 vertices) and 8 points (4 vertices and 4 midpoints) respectively, if the IOU of the 2 polygons grater than a threshold, then we choose the 4 vertices formed polygon, otherwise we will use 8 points to generate a rotation box by the minarearect function in OpenCV.



% we use the algorithm \ref{algorithm2} to generate the final rectangular box.


% \begin{algorithm}
% \caption{Keypoints2Quadrilateral} 
% \hspace*{0.02in} {\bf Input:} 
% 4 corner points $(p_{1}, p_{2}, p_{3}, p_{4})$ \& 4 middle points  \hspace*{0.5in} $(p_{5}, p_{6}, p_{7}, p_{8})$\vspace{0.5ex}\\
% \hspace*{0.02in} {\bf Output:} 
% quadrilateral
% \begin{algorithmic}[1]
% \State $P\gets\{p_{1}, p_{2}, p_{3}, p_{4}\}$;\\
% $P^{'}\gets\{p_{1}, p_{2},p_{3}, p_{4}, p_{5}, p_{6}, p_{7}, p_{8}\}$;\\
% poly1 = $makepolygon(P)$;\\
% poly2 = $minarearect(P)$;\\
% poly3 = $minarearect(P^{'})$;\\
% poly11 = $intersection$ (poly1, poly3);\\
% poly21 = $intersection$ (poly2, poly3);
% \If{poly11.area / poly3.area $>$ threshold}
%     \State return poly1;\\
% \ElseIf \textbf{elseif} {poly21.area / poly3.area $>$ threshold} \textbf{then}
%     \State return poly2;
% \Else
%     \State return poly3;
% \EndIf
% \end{algorithmic}
% \label{algorithm2}
% \end{algorithm}
